FL-WBC: Enhancing Robustness against Model Poisoning Attacks in Federated Learning from a Client Perspective

Federated learning (FL) is a popular distributed learning framework that trains a global model through iterative communications between a central server and edge devices. Recent works have demonstrated that FL is vulnerable to model poisoning attacks. Several server-based defense approaches (e.g. robust aggregation), have been proposed to mitigate such attacks. However, we empirically show that under extremely strong attacks, these defensive methods fail to guarantee the robustness of FL. More importantly, we observe that as long as the global model is polluted, the impact of attacks on the global model will remain in subsequent rounds even if there are no subsequent attacks. In this work, we propose a client-based defense, named White Blood Cell for Federated Learning (FL-WBC), which can mitigate model poisoning attacks that have already polluted the global model. The key idea of FL-WBC is to identify the parameter space where long-lasting attack effect on parameters resides and perturb that space during local training. Furthermore, we derive a certified robustness guarantee against model poisoning attacks and a convergence guarantee to FedAvg after applying our FL-WBC. We conduct experiments on FasionMNIST and CIFAR10 to evaluate the defense against state-of-the-art model poisoning attacks. The results demonstrate that our method can effectively mitigate model poisoning attack impact on the global model within 5 communication rounds with nearly no accuracy drop under both IID and Non-IID settings. Our defense is also complementary to existing server-based robust aggregation approaches and can further improve the robustness of FL under extremely strong attacks.

==> attack_analysis_bak.tex <==
\section{Model Poisoning Attack  in FL} \label{sec:attack_analysis}
To better understand the impact of model poisoning attacks in FL scenarios,  we first need to theoretically analyze how the poisoning attack affects the learning process and provide a mathematical estimation to quantitatively assess the attack effect on model parameters. During this process we come to a deeper understanding of the  reasons for the persistence of the attack effect observed in \S\ref{sec:motivation}. Without loss of generality, we employ FedAvg~\cite{mcmahan2017communication}, the most widely applied FL algorithm as the representative FL method throughout this paper.

 %Based on the quantitative estimator, we analyse that the reason why effective attacks persist in the global model is that the effective attack on parameters resides in the kernels of Hessian matrices of benign objects in FedAvg. Our analysis also demonstrates that all the server-side defense strategies can not efficiently eliminate the attack effect already embedded in the global model. Finally, we conduct experiments to support our analysis.


\subsection{Problem Formulation}

The learning objective of  FedAvg is defined as:

{\small
\begin{equation}
\label{eqn:fedavg}
\mW = \min\limits_{\mW} \{ F(\mW) \triangleq \sum\limits_{k=1}^{N} p^{k} F^{k}(\mW) \},
\end{equation}
}%
where $\mW$ is the weights of the global model, $N$ represents the number of devices, $F^k$ is the local objective of the $k$-th device, $p^k$ is the weight of the $k$-th device, $p^k \geq 0$ and $\sum_{k=1}^N p^{k} = 1$. 


Equation \ref{eqn:fedavg} is solved in an iterative device-server communication fashion. For a given communication round (e.g. the $t$-th), the central server first randomly selects $K$ devices to compose  a set of participating devices $\sS_t$ and then broadcasts the latest global model $\mW_{t-1}$ to these devices. Afterwards, each device (e.g. the $k$-th) in $\sS_t$ performs $I$ iterations of local training using their local data. However, the benign devices and malicious devices perform the local training in different manners.
Specifically, if the $k$-th device is benign, in each iteration (e.g. the $i$-th), the local model $\mW_{t,i}^k$ on the $k$-th device is updated following:
{\small
\begin{equation}
\label{equ:update_benign}
\mW_{t,i+1}^{k} \leftarrow \mW_{t,i}^{k} - {\eta}_{t,i}\nabla F^{k}(\mW_{t,i}^{k},{\xi}_{t,i}^{k}),
%\end{aligned}
\end{equation}
}%
where ${\eta}_{t,i}$ is the learning rate, ${\xi}_{t,i}^{k}$ is a batch of data samples uniformly chosen from the $k$-th device and $\mW_{t,0}^k$ is initialized as $\mW_{t-1}$. In contrast, if the $k$-th device is malicious, the local model $\mW_{t,i}^k$ is updated according to:
{\small
\begin{equation}
\label{equ:mal_update}
\mW_{t,i+1}^{k} \leftarrow \mW_{t,i}^{k} - {\eta}_{t,i}[\alpha \nabla F^{k}(\mW_{t,i}^{k},{\xi}_{t,i}^{k}) +(1-\alpha)\nabla F_{M}(\mW_{t,i}^{k}, {\pi}_{t,i})],
%\end{aligned}
\end{equation}
}%
where $F_M$ is the malicious objective shared by all the malicious devices. $D_M$ is a malicious dataset that consists of the data samples following the same distribution as the benign training data but with adversarial data labels. All the malicious devices share the same malicious dataset $D_M$ and ${\pi}_{t,i}$ is a batch of data samples from $D_M$ used to optimize the malicious objective. Except that they share a malicious dataset, the malicious attackers have the same background knowledge as the benign clients. The goal of the attackers is to make the global model achieve a good performance on the malicious objective (i.e. targeted misclassification on $D_M$). Considering the obliviousness of attack, the malicious devices also optimize benign objective, and the trade-off between the benign and malicious objective is controlled by $\alpha$, where $\alpha\in[0,1]$. Finally, the server averages the local models of the selected $K$ devices and updates the global model as follows:
{\small
\begin{equation}
\label{equ:aggregation}
\mW_{t} \leftarrow \frac{N}{K}\sum\limits_{k \in \sS_t} p^{k} \mW_{t,I}^{k}.
\end{equation}
}%
\subsection{Estimation of Attack Effect on Model Parameters}
Based on the above formulated training process, we analyze the impact of poisoning attacks on model parameters.
To this end, we denote the set of attackers as $\sM$, and introduce a new notation $\mW_t(\sS_i \setminus \sM)$, which represents the global model weights in the $t$-th round when all malicious devices in $\sS_i (i\leq t)$ do not perform the attack in the $i$-th training round. Specifically, when $i = t$, $\mW_t(\sS_t \setminus \sM)$ is optimized following:

{\small
\begin{equation}
\mW_{t}(\sS_t \setminus \sM) \leftarrow \frac{N}{K}\sum\limits_{k \in \sS_t} p^{k} \mW_{t,I}^{k}(\alpha=1),
\end{equation}
}%

where $\mW_{t,I}^{k}(\alpha=1)$ indicates that $\mW_{t,I}^{k}$ is trained  using Equation~\ref{equ:mal_update} with setting $\alpha=1$ (i.e.,  the $k$-th device is benign). A special case is $\mW_t(\sS \setminus \sM)$, which means the global model is optimized when all the malicious devices do not conduct attacks before the $t$-th round. To quantify the attack effect on the global model, we define the Attack Effect on Parameter (AEP) as follows:


\begin{definition}
\label{def:AEP}
Attack Effect on Parameter (AEP), which is denoted as $\delta_t$, is the change of the global model parameters accumulated until $t$-th round due to the attack conducted by the malicious devices in the FL system:
{\small
\begin{equation}
\delta_{t} \triangleq \mW_{t}(\sS \setminus \sM) - \mW_{t}.
\end{equation}
}%
\end{definition}


Based on $AEP$, we can quantitatively  evaluate the attack effect on the malicious objective using $F_M(\mW_{t}(\sS \setminus \sM)-\delta_t)-F_M(\mW_{t}(\sS \setminus \sM)).$ 
As Figure~\ref{fig:defense_baselines} illustrates, although $\mW_{t}(\sS \setminus \sM)$ keeps updating after an adversarial round and there are no more attacks before  the next adversarial round, the attack effect on the global model, i.e., $F_M$ , remains for a number of rounds.
Based on such an observation, we assume that the optimization of malicious objective is dominated by $\delta_t$ compared to $\mW_{t}(\sS \setminus \sM)$, which is learned from the benign objective. Consequently, if the attack effect in round $\tau$ remains for further rounds, $\|\delta_{t+1}-\delta_{t}\|$ should be small for $t\geq \tau.$

To analyze why the attack effect can persist in the global model, we consider the scenario where the malicious devices are selected in round $\tau_1$ and $\tau_2$, but will not be selected between these two rounds. We derive an estimator of $\delta_{t}$ for $\tau_1 < t < \tau_2$, denoted as $\hat{\delta}_{t}$:

{\small
\begin{equation}
\label{eq: est_AEP}
\hat{\delta}_{t} = \frac{N}{K}[\sum\limits_{k \in \sS_t} p^{k} \prod\limits_{i = 0}^{I-1}{(\mI - \eta_{t,i}\mH_{t,i}^k)}] \hat{\delta}_{t-1},
\end{equation}
}%
where $\mH_{t,i}^k \triangleq \nabla^2 F^{k}(\mW_{t,i}^{k},{\xi}_{t,i}^{k}).$ The derivation process is presented in Appendix \ref{app:est_AEP}. Note that, we do not restrict the detailed malicious objective during derivation, and thus our estimator and analysis can be extended to other attacks, such as backdoor attacks.

\subsection{Unveil Long-lasting Attack Effect}\label{sec:unveil_attack}

The key observation from Equation \ref{eq: est_AEP} is that if $\hat{\delta}_{\tau}$ is in the kernel of each $\mH_{t,i}^k$ for $i$-th iteration where $k\in \sS_t$ and $t > \tau$, then $\hat{\delta}_{t}$ will be the same as $\hat{\delta}_{\tau}$, which keeps $AEP$ in the global model. 
Based on this observation, we discover that {\bf{the reason why attack effects remain in the aggregated model is that the $AEP$s  reside in the kernel of $\mH_{t,i}^k$.}} 
To validate our analysis, we conduct experiments on Fashion-MNIST with model poisoning attacks in FL. The experiment details and results are shown in Appendix \ref{app:exp_4.3}. The results show that $\|\mH_{t,i}^k \delta_t \|_2$ would be nearly 0 under effective attacks. We also implement attack boosting by regularizing $\delta_t$ to be in the kernel of $\mH_{t,i}^k$. 
% \makeatletter\def\@captype{figure}\makeatother
% \begin{minipage}[b]{.38\textwidth}
% \centering
%      \includegraphics[scale=0.40]{images/unveil_attack.eps}
% \label{fig:unveil_attack}
% \caption{Compared results of misclassification loss on malicious dataset for model poisoning attack with and without applying $R_H$. The black circle denotes the adversarial rounds.}
% \end{minipage}
% \makeatletter\def\@captype{table}\makeatother
% \begin{minipage}[b]{.6\textwidth}
% \centering
% \begin{tabular}{c||c|c}
%   \toprule
%   Adversarial round & baseline $\Phi_t$ & $\Phi_t$ applying $R_H$\\
%   \hline
%   5 & 3.56 & 1.06\\
%   \hline
%   11 & 0.00 & 0.00\\
%   \hline
%   26 & 0.01 & 0.00\\
%   \hline
%   32 & 0.00 & 0.00\\
%   \hline
%   48 & 0.00 & 0.00\\
%   \hline
%   60 & 0.05 & 0.00\\
%   \hline
%   67 & 0.07 & 0.00\\
%   \hline
%   76 & 0.00 & 0.00\\
%   \hline
%   83 & 0.00 & 0.00\\
%   \hline
%   93 & 0.00 & 0.00\\
%   \bottomrule
% \end{tabular}
% \label{table:unveil_attack}
% \caption{Numerical results of $\Phi_t$ with and without applying $R_H$ at adversarial rounds.}
% \end{minipage}


% To validate our analysis, we conduct experiments on Fashion-MNIST with model poisoning attacks in FL training. Considering the high computation overhead for calculating $\mH_{t,i}^k$, we first approximate $\mathbb{E}_{i\in[I], k\in \sS_t \setminus \sM} (\mH_{t+1,i}^k \delta_t)$ denoted as $\Phi_t$  for each round $t$ when the malicious devices are involved in training. The detailed experiment settings and how we compute $\Phi_t$ can be found in Appendix \ref{}. 
% The results of baseline in Figure \ref{fig:unveil_attack} shows the loss that the malicious data is miss-classified by the global model, and the computed $\Phi_t$ for each adversarial round is presented in Table \ref{table:unveil_attack}. The results show that for the first adversarial round (i.e. round 5), the value of $\Phi_t$ is higher than 3 and the attack is mitigated rapidly. While for the following adversarial rounds, $\Phi_t$s are nearly 0, and the miss-classification loss keeps low until the next attack is conducted. This result is consistent with our above analysis for why  attack effects can remain in the aggregated model. In addition, we introduce a regularization $R_H$ that approximates $\|\mH_{t,i}^k \delta_t \|_2$ into the local training of malicious devices, enforcing $\delta_t$ to reside in the null space of $\mH_{t,i}^k$. We aim to evaluate  whether the poisoning attack can be boosted after applying $R_H$, i.e., the attack effect remains for more rounds. The detailed formulation of $R_H$ can be found in Appendix \ref{}. As  Figure \ref{fig:unveil_attack} and Table~\ref{table:unveil_attack} show, the values of $\Phi_t$ in round 5, 60 and 67 are reduced after applying $R_H$ and the corresponding attacks are boosted. This result further supports our analysis that the reason why effective attacks can remain in the aggregated model is that the $AEP$s reside in the kernels of $\mH_{t,i}^k$. 
% %Additionally, we observe that with the convergence of the benign task, $\mH_{t,i}^k$ would have more than 50\% elements to be 0. This extremely high sparsity of $\mH_{t,i}^k$ tends to leading to low rank, which is equal to high dimension of the kernel of $\mH_{t,i}^k$, and increases the vulnerability that $AEP$s would be hidden in $\mH_{t,i}^k$'s kernel.



The above theoretical analysis and experiment results suggest that all the server-based defense methods (e.g. robust aggregation) will not be able efficiently mitigate the impact of model poisoning attacks to the victim global model. The fundamental reason for the failure of these mitigations is that: \textbf{the transmission of $AEP$ $\delta_t$ in global model is determined by $\mH_{t,i}^k$, which is inaccessible by the central server.} Therefore, it is necessary to design an effective defense mechanism at client side aiming at mitigating attack that has already polluted the global model to further enhance the robustness of FL.

==> design_bak.tex <==
\section{FL-WBC} \label{sec:design}

\subsection{Defense Formulation}
Our aforementioned analysis shows that $AEP$ resides in the kernels of the Hessian matrix that is generated during the benign device's local training. In this section, we propose \textit{White Blood Cell for Federated Learning (FL-WBC)} to  efficiently mitigate the attack effect on the global model. In particular, we reform the local model training of benign devices to achieve two goals:

\begin{itemize}
    \item Goal 1: To maintain the benign task's performance, loss of local benign task should be minimized.
    
    \item Goal 2: To prevent $AEP$ from being hidden in the kernel of  Hessian matrices on benign devices, the rank of $\mH_{t+1,i}^k$ should be maximized, which is equivalent to minimize the dimension of $\mH_{t+1,i}^k$'s kernel.
\end{itemize}

Performing regularization on $\mH_{t,i}^k$ is helpful for squeezing the dimension of $\mH_{t+1,i}^k$'s kernel. However, it is computationally unaffordable to perform the  regularization on $\mH_{t,i}^k$ due to its high dimensions.
Therefore, in order to achieve Goal 2, we consider the essence of $\mH_{t,i}^k$, i.e., second-order partial derivatives of the loss function, where the diagonal elements describe the change of gradients $\nabla F^{k}(\mW_{t,i+1}^{k}) - \nabla F^{k}(\mW_{t,i}^{k})$ across iterations. We assume a fixed learning rate is applied for each communication round, and then $\nabla F^{k}(\mW_{t,i+1}^{k}) - \nabla F^{k}(\mW_{t,i}^{k})$ can be approximated by $(\Delta \mW_{t,i+1}^k - \Delta \mW_{t,i}^k)/\eta_{t,i}$.
In the experiments presented in \S4.3, we observe that $\mH_{t,i}^k$  has more than 60\% elements to be zero in the most of iterations. When $\mH_{t,i}^k$ is highly sparse, we set its diagonal, which is approximately $(\Delta \mW_{t,i+1}^k - \Delta \mW_{t,i}^k)/\eta_{t,i}$, to be non-zero for increasing the rank of $\mH_{t,i}^k$. Formally, we have the following objective functions with respect to $\mW$ to optimize $\mW_{t,i+1}^k$:

\begin{align}
    &\textrm{\bf Achieving Goal 1: } \min\limits_{\mW} F^{k}(\mW), \label{equ:goal1} \\
    &\textrm{\bf Achieving Goal 2: } \max\limits_{\mW} \| ReLU(| (\mW-\mW_{t,i}^k) - \Delta \mW_{t,i}^k|/\eta_{t,i}-|\Upsilon|) \|_0, \label{equ:goal2}
\end{align}
where $\Upsilon$ is a threshold matrix with the same shape of $\mW$, we apply it as the lower bound of the magnitude of elements in $(\Delta \mW_{t,i+1}^k - \Delta \mW_{t,i}^k)/\eta_{t,i}$.

\subsection{Defense Solution}

Considering that objective of Goal 2 is non-differentiable, we apply Proximal Gradient Decent~\cite{nesterov2003introductory} for optimization. We apply gradient decent to achieve Goal 1 and the proximal operator to solve Goal 2. Formally, we have two steps to optimize $\mW_{t,i+1}^k$:

{\small
   \begin{align}
    &\hat{\mW_{t,i+1}^{k}} = \mW_{t,i}^{k} - {\eta}_{t,i}\nabla F^{k}(\mW_{t,i}^{k},{\xi}_{t,i}^{k}), \label{equ:main_obj} \\
     &\mW_{t,i+1}^{k}=\arg\min\limits_{\mW} [-\lambda\| ReLU(| (\mW-\mW_{t,i}^k) - \Delta \mW_{t,i}^k|/\eta_{t,i}-|\Upsilon| )\|_0 + \frac{1}{2}\|\mW - \hat{\mW_{t,i+1}^{k}}\|_2], \label{equ:prox_obj}
\end{align} 
}%


where $\lambda$ in Equation~\ref{equ:prox_obj} controls the trade-off between the objective of proximal operator and the smoothness of convergence. In this work, we set $\lambda=\infty$ to guarantee the effectiveness of proposed defense effect, and hence Equation~\ref{equ:prox_obj} can be  rewritten as:

{\small
\begin{align}
    &\mW_{t,i+1}^{k}=\arg\min\limits_{\mW} \|\mW - \hat{\mW_{t,i+1}^{k}}\|_2,\\
   & s.t.\| ReLU(| (\mW-\mW_{t,i}^k) - \Delta \mW_{t,i}^k|/\eta_{t,i}-|\Upsilon|) \|_0 = SZ_{\mW},
\end{align}
}%
where $SZ_{\mW}$ denotes the number of elements in $\mW$. Note that we have different choices of $\Upsilon$. In this work, we set $\Upsilon$ as Laplace noise with $mean=0$ and $std=s$, since the randomness of $\Upsilon$ will make attackers harder to determine the defense strategy. Specifically, our defense is to find the elements in $\hat{\mW_{t,i+1}^{k}}$ whose corresponding values in $| (\hat{\mW_{t,i+1}^{k}}-\mW_{t,i}^k) - \Delta \mW_{t,i}^k|/\eta_{t,i}$ are smaller than the counterpart in $\Upsilon$. The detailed algorithm describing the local training process on benign devices when applying FL-WBC can be found in Appendix \ref{app:alg}.

% \begin{algorithm}[t]  
% \footnotesize
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
%     \caption{Local training process applying FL-WBC on a benign device in round $t$. }
%     \label{alg:Framwork}  
%     \begin{algorithmic}[1] 
%         \Require Local training data $\sD \in \sR^{L\times M\times N}$; Local objective function $F: \sR^{M\times N} \rightarrow \sR$; Local model parameters $\mW \in \sR^{M\times N}$; The number of local training epochs $E$; Learning rates $\eta_{t,i}$ for $i\in [E]$; Threshold matrix $\Upsilon \in \sR^{M\times N}$. 
%         \Ensure Learnt model parameter $\mW$ with our defense.
%         \State Initialize $\mW$;
%         \State Initialize $\mW_{-2}$
%         \For {$i\in[E]$}
%             \For {batch $\sB$ in $\sD$}
%                 \State $\mW_{-1} \leftarrow \mW$;
%                 \State $\mW \leftarrow \mW - \eta_{t,i} F(\mW, \sB)$;
%                 \If {this is not the first training batch}
%                     \State $\mW^* \leftarrow (\mW - \mW_{-1})-(\mW_{-1}-\mW_{-2})$;
%                     \State Find the set $\mathbb{S}$ which contains the indices of elements in $|\mW^*|-\eta_{t,i}|\Upsilon|$ which are less than 0;
%                     \For{${i,j} \in \sS$}
%                         \If {$\mW^* \geq 0$}
%                             \State $\mW \leftarrow \mW + \eta_{t,i}|\Upsilon|-|\mW^*|$;
%                         \Else 
%                             \State $\mW \leftarrow \mW + |\mW^*| - \eta_{t,i}|\Upsilon|$;
%                         \EndIf
%                     \EndFor
%                 \EndIf
%                 \State $\mW_{-2} \leftarrow \mW_{-1}$;
%             \EndFor
%         \EndFor
        
%     \end{algorithmic} \label{alg:FL-WBC}
% \end{algorithm} 

\subsection{Certified Robustness Guarantee}
We define our {\textit{certified robustness guarantee}} as the distance of $AEP$ between the adversarial round and the subsequent rounds where  FL-WBC is applied. A larger distance of $AEP$ indicates that FL-WBC can mitigate the attack  more efficiently. We first make an assumption for the Hessian matrix after applying our defense:

\begin{assumption} \label{asm:hessian}

After applying FL-WBC, the new benign training Hessian matrix $H'$ would be nearly full-rank. Following the notation of $s$ as the variance of $\Upsilon$ in Equation~\ref{equ:prox_obj}, the operator $H'$ is bounded below: $\mathbb{E} \|H'\va\|_2^2/P \geq s\|\va\|_2^2.$

\end{assumption}

Additionally, we make assumptions on bounding the norm of $AEP$s in different rounds and independent distributions of $H_{t,i}^k\delta_{t,i}^k$.

\begin{assumption} \label{asm:aep_norm}

The expected norm of $AEP$s is lower bounded in each round across devices and iterations: $\mathbb{E}_{i\in [I], k \in \sS_t} \|\delta_{t, i}^k\|_2^2 \geq \Lambda_t.$

\end{assumption}

% \begin{assumption} \label{asm:aep_divergence}

% Applying the same $\Upsilon$, the divergence of $AEP$ changing is bounded in different rounds across devices and iterations: $\frac{\|\Delta \delta_{t_1, i_1}^{k_1} + \Delta \delta_{t_2, i_2}^{k_2} \|_2}{\|\Delta \delta_{t_1, i_1}^{k_1}\|_2 + \|\Delta \delta_{t_2, i_2}^{k_2}\|_2} \geq J . $

% \end{assumption}



\begin{assumption} \label{asm:aep_divergence}

Since local training data have independent distributions, the elements in $H_{t,i}^k\delta_{t,i}^k$ are independent and have expectations of 0 in different rounds across devices and iterations.

\end{assumption}

Following the notations in \S\ref{sec:attack_analysis} and applying the local training of benign devices in Algorithm~\ref{alg:FL-WBC}, which can be found in Appendix \ref{app:alg}, we have the following theorem for our {\textit{robustness guarantee}} on FedAvg after applying FL-WBC.

\begin{theorem}
\label{thm:robustness}
Let Assumption \ref{asm:hessian}-\ref{asm:aep_divergence} hold and $s, \Lambda_t, P$ be defined therein. $K$ denotes the number of devices involved in training for each round. Assuming that poisoning attack happens in round $t_{adv}$ and no attack happens from round $t_{adv}$ to $T$, then for FedAvg applying FL-WBC we have:

{\small
\begin{equation}
    \mathbb{E} \|\hat{\delta}_T - \hat{\delta}_{t_{adv}} \|_2^2 \geq \frac{P I s}{K} \sum\limits_{t=t_{adv}+1}^{T} \eta_{t,I-1}^2\Lambda_t.
\end{equation}
}%


\end{theorem}

\begin{proof}
See our proof in Appendix~\ref{app:robustness}.
\end{proof}




==> evaluation_bak.tex <==
\section{Experiments} \label{sec:evaluation}

In our experiments, we evaluate FL-WBC against targeted model poisoning attack \cite{bhagoji2019analyzing} described in \S\ref{sec:attack_analysis} under both IID and non-IID settings. Experiments are conducted on a server with two Intel Xeon E5-2687W CPUs and four Nvidia TITAN RTX GPUs.

\subsection{Experimental Setup}
\vspace{-1.5mm}

\paragraph{Attack method.}

We evaluate our defense against model poisoning attack shown in \cite{bhagoji2019analyzing,tomsett2019model}. There are several attackers in FL setup and all the attackers share a malicious dataset $D_M$, whose data points obey the same distribution with benign training data while having adversarial labels. We let all the attackers conduct the model poisoning attack at adversarial rounds $t_{adv}$ simultaneously such that the attack will be extremely strong. 

\vspace{-3.5mm}
\paragraph{Defense baseline.}

We compare our proposed defense with two categories of defense methods that have been widely used: (1) \textbf{Differential privacy (DP)} improves robustness with theoretical guarantee by clipping the gradient norm and injecting perturbations to the gradients.  We adopt both \textbf{Central Differential privacy (CDP)}~\cite{naseri2020toward} and \textbf{Local Differential privacy (LDP)}~\cite{naseri2020toward} for comparisons. We set the clipping norm as 5 and 10 for Fashion-MNIST and CIFAR10 respectively following~\cite{naseri2020toward} and apply Laplace noise with $mean=0$ and $variance=\sigma_{dp}$.
(2) \textbf{Robust aggregation} improves robustness of FL by manipulating aggregation rules. We consider both \textbf{Coordinate Median Aggregation (CMA)}~\cite{yin2018byzantine} and \textbf{Coordinate Trimmed-Mean Aggregation (CTMA)}~\cite{yin2018byzantine} as baselines.

\vspace{-3.5mm}

\paragraph{Datasets.}

To evaluate our defense under more realistic FL settings, we construct IID/non-IID datasets based on Fashion-MNIST and CIFAR10 by following the configurations in~\cite{mcmahan2017communication}. The detailed data preparation can be found in Appendix \ref{app:exp_setup}. We sample 1 and 10 images from both datasets to construct the malicious dataset $D_{M}$ corresponding to scenarios $D_M$ having single image and multiple images. Note that, data samples in $D_M$ would not appear in training datasets of benign devices.

\vspace{-3.5mm}
\paragraph{Hyperparameter configurations.}

%For training, we set local epoch $E$ as 1 and batch size $B$ as 32. We apply SGD optimizer and set the learning rate $\eta$ to 0.01. We set 5 devices out of totally 100 devices to be malicious. 
Each communication round is set to be the adversarial round with probability 0.1. In each benign communication round, there are 10 benign devices which are randomly selected to participate in the training. In each adversarial round, 5 malicious and 5 randomly selected benign devices participate in the training, which means there  are 50\% attackers involved in adversarial rounds. Additional configurations and model structures can be found in Appendix \ref{app:exp_setup}.

\vspace{-3.5mm}
\paragraph{Evaluation metrics.} (1) {\bf Attack metric (Misclassification confidence/accuracy:)} We define misclssification confidence/accuracy as the classification confidence/accuracy of the global model on the malicious dataset.
%for the scenarios $D_M$ having single and multiple images respectively.  
(2) {\bf Robust metric (Attack mitigation rounds):} We define \textit{attack mitigation rounds} as the number of communication rounds after which the misclassification confidence can decrease to lower than 50\% or misclassification accuracy can decrease to lower than the error rate for the benign task. %for the scenarios $D_M$ having single and multiple images respectively. 
(3) {\bf Utility metric (Benign accuracy):} We use the accuracy of the global model on the benign testing set of the primary task to measure the effectiveness of FL algorithms (i.e., FedAvg~\cite{mcmahan2017communication}). The higher the accuracy is, the higher utility is obtained.

%\subsection{Effectiveness of FL-WBC with \textit{Single} Image in The Malicious Dataset}
\subsection{Experimental Results}

\begin{figure*}[t]
\centering
     \includegraphics[scale=0.30]{images/misclassification_round.eps}
\caption{Comparison of  misclassification confidence and communication round on FashionMNIST and CIFAR-10 with IID/non-IID settings. The black circle denotes the adversarial rounds.}
\label{fig:misacc_round}
\end{figure*}

\begin{figure*}[t]
\centering
     \includegraphics[scale=0.30]{images/acc_mitigation_single.eps}
\caption{Comparison of  benign accuracy and attack mitigation rounds on  FashionMNIST and CIFAR-10 with IID/non-IID settings when $D_M$ has only one image.}
\label{fig:acc_mitigation_single}
\end{figure*}

We first show the results when there is only one image in the malicious dataset. We consider IID and non-IID settings for both Fashion-MNIST and CIFAR10 datasets. Figure~\ref{fig:misacc_round} shows the misclassification confidence of our defense and the robust aggregation baselines in the first 60 communication rounds. The results show that our defense can more effectively and efficiently  mitigate the impact of model poisoning attack in comparison with baseline methods. In particular, FL-WBC can mitigate the impact of model poisoning attack within 5 communication round when $s$ (i.e., variance for $\Upsilon$) is 0.4 for both IID and non-IID settings. With regard to CMA and CTMA, the attack impact can not be mitigated within 10 subsequent rounds even when $\beta$ for CTMA is 0.4, where 80\% of local updates are trimmed before aggregation. Thus, the robust aggregation baselines fail to mitigate the model poisoning attack under our attack settings.


%For IID settings, the results show that FL-WBC can mitigate the impact of model poisoning attack in one communication round when $s$ (i.e., variance for $\Upsilon$) is 0.4. The global model suffers nearly no degradation on accuracy when applying this level of defense. With regard to CDP, attack impact can not be mitigated within  10 subsequent rounds when $var_{DP}$ (i.e., the variance of Laplace noise) is 1. The benign accuracy of the global model shows obvious drop adding such level of noise. 
%Defense becomes much harder for Non-IID setting. Our defense can still guarantee that the attack impact would be mitigated in 5 rounds with less than 5\% drop on benign accuracy when $s=0.4$ for both datasets. For CDP, it can not be guaranteed that the attack impact can be mitigated within 5 rounds even when $Var_{DP}=10$ while the benign accuracy of the global model suffers more than 30\% drop under such level of noise. The reason why defense for non-IID settings is harder is that the devices train only a part of parameters\cite{li2020lotteryfl} when holding only a few classes of data and leads to a sparser $H_{t,i}^k$, which is more likely to have a kernel with higher dimension.

We also compare our defense with CDP and LDP in terms of \textit{benign accuracy} and \textit{attack mitigation rounds}. We evaluate our defense by  varying $s$ from 0.1 to 1, and evaluate DP baselines by changing $\sigma_{dp}$ from 0.1 to 10. For each defense method, we show the trade-off between \textit{benign accuracy} and \textit{attack mitigation rounds} in Figure \ref{fig:acc_mitigation_single}. We have two key observations: 1) With sacrificing less than 5\% benign accuracy, FL-WBC can mitigate the impact of model poisoning attack  on the global model in 1 communication round for IID settings, and within 5 communication rounds for non-IID settings respectively. However,  CDP and LDP fail to mitigate attack effect within 5 rounds for IID and within 10 rounds for non-IID settings with less than 5\% accuracy drop. 2) For non-IID settings where the defense becomes more challenging, FL-WBC can still mitigate the attack effect within 2 rounds with less than 15\% benign accuracy drop, but DP can not make an effective mitigation within 3 rounds with less than 30\% benign accuracy drop, leading to the unacceptable utility on the benign task. The reason of FL-WBC outperforming CDP and LDP is that FL-WBC only inject perturbations to the parameter space where the long-lasting $AEP$ resides in instead of perturbing all the parameters like DP methods. Therefore,  FL-WBC can achieve better robustness with less accuracy drop. 

In addition, we also observe that defense for non-IID settings is harder than IID settings,  the reason is that  under non-IID settings the devices train only a part of parameters~\cite{li2020lotteryfl} when holding only a few classes of data, leading to a sparser $H_{t,i}^k$ that is more likely to have a kernel with a higher dimension.

We also perform evaluations on the malicious dataset which consists of multiple images, and conduct experiments by integrating the robustness aggregation with FL-WBC to demonstrate that  FL-WBC is complementary to server-based defenses. The detailed results are presented in Appendix \ref{app:exp:WBC}. 
%The results when there are multiple images in the malicious dataset can be found in Appendix \ref{app:exp:WBC}. We also conduct experiments applying both robustness aggregation and FL-WBC to show that our FL-WBC is complementary to server-based defenses. The results can be found in Appendix \ref{app:exp:WBC}.





